Estimation of the parameters of the Ornstein-Uhlenbeck's stochastic process

It is considered Ornstein-Uhlenbeck process $ x_t = x_0 e^{-\theta t} + \mu (1-e^{-\theta t}) + \sigma \int_0^t e^{-\theta (t-s)} dW_s$, where $x_0 \in R$, $\theta>0$, $ \mu \in R$ and $\sigma > 0$ are parameters. By use values $(z_k)_{k \in N}$ of corresponding trajectories at a fixed positive moment $t$, a consistent estimate of each unknown parameter of the Ornstein-Uhlenbeck's stochastic process is constructed under assumption that all another parameters are known.

==> tsp-short.cls.tex <==
%%
%% LaTeX documentclass for the journal
%%	Theory of Stochastic Processes
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%<identification>%
\NeedsTeXFormat{LaTeX2e}
	[2001/06/01]
\ProvidesClass{tsp-short}
	[2009/02/03 v1.11 TSP Author Class]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%<Options>%
\ProcessOptions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%<Package load>%
\RequirePackage[english]{babel}

\LoadClass{amsart}[1999/11/24]

\RequirePackage{amssymb}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%<Main code>%
%% Default language
\selectlanguage{english}

%% Set margins
\textwidth=32pc
\textheight=52.5pc

\setlength{\oddsidemargin}{0pt}
\setlength{\evensidemargin}{0pt}
\setlength{\topmargin}{-2pt}
\addtolength{\textheight}{10pt}
%%
\endinput

